Benchmarking News Recommendation in the Era of Green AI

Over recent years, news recommender systems have gained significant attention in both academia and industry, emphasizing the need for a standardized benchmark to evaluate and compare the performance of these systems. Concurrently, Green AI advocates for reducing the energy consumption and environmental impact of machine learning. To address these concerns, we introduce the first Green AI benchmarking framework for news recommendation, known as GreenRec, and propose a metric for assessing the tradeoff between recommendation accuracy and efficiency. Our benchmark encompasses 30 base models and their variants, covering traditional end-to-end training paradigms as well as our proposed efficient only-encode-once (OLEO) paradigm. Through experiments consuming 2000 GPU hours, we observe that the OLEO paradigm achieves competitive accuracy compared to state-of-the-art end-to-end paradigms and delivers up to a 2992\% improvement in sustainability metrics.

==> Plots/carbon-size/main.tex <==
\definecolor{zhucao}{rgb}{0.65, 0.25, 0.21}
\definecolor{fuguang}{rgb}{0.94, 0.76, 0.64}
\definecolor{tushoulan}{rgb}{0.50, 0.76, 0.89}
\definecolor{qingdai}{rgb}{0.51, 0.72, 0.61}


\begin{figure}
\centering
\setlength\tabcolsep{0pt}

\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c}

\begin{tikzpicture}

    \begin{groupplot}[
        group style={
            group name=my fancy plots,
            group size=1 by 2,
            xticklabels at=edge bottom,
            vertical sep=0pt
        },
        width=12cm,
        % line width=0.35mm,
        xtick={0, 5000, 10000, 15000, 20000, 25000, 30000},
        xticklabels={0, 5, 10, 16, 20, 25, 30},
        xmin=0,
        xmax=30000,
        xlabel=Carbon Emission (Kg),
        ylabel=AUC,
        xmajorgrids=true,
        ymajorgrids=true,
        grid style=dashed,
        legend columns=2,
        legend style={
            font=\normalsize,
            legend cell align=left,
        },
        legend pos=south east,
    ]
    
    \nextgroupplot[
        ymin=63,
        ymax=66,
        ytick={64, 66},
        axis x line=top, 
        axis y discontinuity=parallel,
        height=4.5cm,
        xlabel=,
        y label style={at={(-0.1,0.1)}},
    ]
        % NRMS
        \addplot[color=fuguang, only marks, style={mark=*, fill=fuguang,mark size=4pt}] coordinates {(1010,64.12)};\label{plot:nrms}
        % \addlegendentry{}
        % DCN
        \addplot[color=fuguang, only marks, style={mark=triangle*, fill=fuguang,mark size=5pt}] coordinates {(972,63.88)};\label{plot:dcn}
        % \addlegendentry{$\texttt{Text-based}$}
        
        % NRMS-PLMNR
        \addplot[color=qingdai, only marks, style={mark=*, 
        fill=qingdai,mark size=4pt}] coordinates {(4043,65.57)};\label{plot:nrms-plm}
        % \addlegendentry{}
        % DCN-PLMNR
        \addplot[color=qingdai, only marks, style={mark=triangle*, fill=qingdai,mark size=5pt}] coordinates {(27036,65.42)};\label{plot:dcn-plm}
        % \addlegendentry{$\texttt{PLM-plugged}$}
        
        % NRMS-MFT
        \addplot[color=zhucao, only marks, style={mark=*, fill=zhucao,mark size=4pt}] coordinates {(505,64.34)};\label{plot:nrms-gnrs}
        % \addlegendentry{}
        % DCN-MFT
        \addplot[color=zhucao, only marks, style={mark=triangle*, fill=zhucao,mark size=5pt}] coordinates {(956,65.44)};\label{plot:dcn-gnrs}
        % \addlegendentry{$\texttt{GNR-based}$}      
    
    \nextgroupplot[
        ymin=56,ymax=58,
        ytick={56, 58},
        axis x line=bottom,
        height=3.0cm,
        ylabel=,
    ]
        % NRMS-id
        \addplot[color=tushoulan, only marks, style={mark=*, fill=tushoulan,mark size=4pt}] coordinates {(471,57.59)}; \label{plot:nrms-id}
        % \addlegendentry{}
        % DCN-id
        \addplot[color=tushoulan, only marks, style={mark=triangle*, fill=tushoulan,mark size=5pt}] coordinates {(926,57.41)};\label{plot:dcn-id}
        % \addlegendentry{$\texttt{ID-based}$}
    \end{groupplot}
    
        \node[draw,fill=white,inner sep=4pt,above left=0.5em] at (6.7, -2.4) {
        \setlength\tabcolsep{2pt}
        \begin{tabular}{ccl}
        $\texttt{NRMS}$ & $\texttt{DCN}$ \\
        \ref{plot:nrms-id} & \ref{plot:dcn-id} & $\texttt{ID-based}$\\
        \ref{plot:nrms} & \ref{plot:dcn} & $\texttt{Text-based}$\\
        \ref{plot:nrms-plm} & \ref{plot:dcn-plm} & $\texttt{PLM-NR}$ \\
        \ref{plot:nrms-gnrs} & \ref{plot:dcn-gnrs} & $\texttt{PREC}$
        \end{tabular}
        };
\end{tikzpicture}
\end{tabular}
}
\caption{\label{fig:example} AUC and carbon emission (\ce) of two popular news recommendation methods NRMS and DCN under different training frameworks on the MIND-large dataset.}
\end{figure}


==> Plots/param/appearance.tex <==

\begin{tikzpicture}

    \begin{groupplot}[
        group style={
            group name=my fancy plots,
            group size=1 by 2,
            xticklabels at=edge bottom,
            vertical sep=0pt
        },
        width=8.5cm,
        % line width=0.35mm,
        xtick={0, 2000, 4000, 6000},
        xticklabels={0, 2, 4, 6},
        xmin=0,
        xmax=7000,
        xlabel=Carbon Emission (Kg),
        ylabel=AUC,
        xmajorgrids=true,
        ymajorgrids=true,
        grid style=dashed,
        legend columns=2,
        legend style={
            font=\normalsize,
            legend cell align=left,
        },
        legend pos=south east,
    ]
    
    \nextgroupplot[
        ymin=63,
        ymax=66,
        ytick={64, 66},
        axis x line=top, 
        axis y discontinuity=parallel,
        height=6.0cm,
        xlabel=,
        y label style={at={(-0.1,0.1)}},
    ]
        % NRMS
        \addplot[color=fuguang, only marks, style={mark=*, fill=fuguang,mark size=4pt}] coordinates {(1010,64.12)};\label{plot:nrms}
        % \addlegendentry{}
        % DCN
        \addplot[color=fuguang, only marks, style={mark=triangle*, fill=fuguang,mark size=5pt}] coordinates {(1684,63.88)};\label{plot:dcn}
        % \addlegendentry{$\texttt{Text-based}$}
        
        % NRMS-PLMNR
        \addplot[color=qingdai, only marks, style={mark=*, 
        fill=qingdai,mark size=4pt}] coordinates {(4043,65.57)};\label{plot:nrms-plm}
        % \addlegendentry{}
        % DCN-PLMNR
        \addplot[color=qingdai, only marks, style={mark=triangle*, fill=qingdai,mark size=5pt}] coordinates {(6570,65.42)};\label{plot:dcn-plm}
        % \addlegendentry{$\texttt{PLM-plugged}$}
        
        % NRMS-MFT
        \addplot[color=zhucao, only marks, style={mark=*, fill=zhucao,mark size=4pt}] coordinates {(505,64.34)};\label{plot:nrms-gnrs}
        % \addlegendentry{}
        % DCN-MFT
        \addplot[color=zhucao, only marks, style={mark=triangle*, fill=zhucao,mark size=5pt}] coordinates {(1010,65.44)};\label{plot:dcn-gnrs}
        % \addlegendentry{$\texttt{GNR-based}$}      
    
    \nextgroupplot[
        ymin=56,ymax=58,
        ytick={56, 58},
        axis x line=bottom,
        height=4.0cm,
        ylabel=,
    ]
        % NRMS-id
        \addplot[color=tushoulan, only marks, style={mark=*, fill=tushoulan,mark size=4pt}] coordinates {(471,57.59)}; \label{plot:nrms-id}
        % \addlegendentry{}
        % DCN-id
        \addplot[color=tushoulan, only marks, style={mark=triangle*, fill=tushoulan,mark size=5pt}] coordinates {(791,57.41)};\label{plot:dcn-id}
        % \addlegendentry{$\texttt{ID-based}$}
    \end{groupplot}
    
        \node[draw,fill=white,inner sep=4pt,above left=0.5em] at (6.7, -2.4) {
        \setlength\tabcolsep{2pt}
        \begin{tabular}{ccl}
        $\texttt{NRMS}$ & $\texttt{DCN}$ \\
        \ref{plot:nrms-id} & \ref{plot:dcn-id} & $\texttt{ID-based}$\\
        \ref{plot:nrms} & \ref{plot:dcn} & $\texttt{Text-based}$\\
        \ref{plot:nrms-plm} & \ref{plot:dcn-plm} & $\texttt{PLM-based}$ \\
        \ref{plot:nrms-gnrs} & \ref{plot:dcn-gnrs} & $\texttt{GNR \small{(ours)}}$
        \end{tabular}
        };
\end{tikzpicture}


==> Plots/param/encoder.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar,
    xtick=data,
    xticklabels={\small{DCN}, \small{DIN}, \small{BST}, \small{LSTUR}, \small{NAML}, \small{NRMS}, \small{PLMNR-LSTUR}, \small{PLMNR-NAML}, \small{PLMNR-NRMS}},
    ylabel=News Encoder Parameter \%,
%    xlabel=Models,
    enlarge x limits=0.15,
    xticklabel style={rotate=45, anchor=east},
    grid=both,
    grid style=dashed,
]
\addplot[lightc!80!black, fill=lightc!80!white] coordinates {(1,0) (2,0) (3,0) (4,27) (5,80) (6,50) (7,96) (8,99) (9,96)};
\end{axis}
\end{tikzpicture}

==> Plots/param/main.tex <==
% \definecolor{lightc}{rgb}{0.86, 0.90, 0.94}

% \begin{figure}
%     \centering
%     \setlength\tabcolsep{0pt}
%     \begin{tabular}{c}
%     \begin{subfigure}{0.4\textwidth}
%         \resizebox{1.0\linewidth}{!}{
%             \input{plots/param/appearance}
%         }
%         \caption{\label{fig:appearance}}
%     \end{subfigure} \\
%     \begin{subfigure}{0.35\textwidth}
%         \resizebox{1.0\linewidth}{!}{
%             \input{plots/param/encoder}
%         }
%         \caption{\label{fig:param}}
%     \end{subfigure}
%     \end{tabular}
    
%     \caption{(a) The relation between news appearance times and proportion of news articles. Each point (x, y) represents y \% of news articles appear less than x times within a training epoch. The line ends at the point (550700, 100). (b) Proportion of parameters occupied by different news encoders in various recommendation models.}
% \end{figure}


==> Plots/percentage/main.tex <==
% \definecolor{lightc}{rgb}{0.86, 0.90, 0.94}

% % \begin{figure}[t]
% % \centering
% % \setlength\tabcolsep{0pt}

% % \resizebox{0.6\linewidth}{!}{
% % \begin{tabular}{c}

% \begin{tikzpicture}
%     \begin{axis}[
%         ylabel=News Articles \%,
%         xlabel=$\#Appearance$,
%         line width=0.35mm,
%         grid=both,
%         grid style=dashed,
%     ]

%         \draw[
%             purple!80!white,
%             dashed,
%             line width=0.6mm,
%             opacity=0.7
%         ] (1818,28) -- (1818,95) node[right] at (2000, 50) {\small{Average appearance: 1818 times}};
        
%         \addplot[
%             lightc!80!black,
%             line width=1mm,
%             % opacity=0.7
%             % mark=x,
%         ] % lifestyle
%             coordinates{
%                 (100, 27.94)
%                 (200, 59.58)
%                 (300, 66.36)
%                 (400, 70.75)
%                 (500, 73.94)
%                 (600, 76.34)
%                 (700, 78.17)
%                 (800, 79.60)
%                 (900, 80.70)
%                 (1000, 81.74)
%                 (1100, 82.57)
%                 (1200, 83.30)
%                 (1300, 84.02)
%                 (1400, 84.64)
%                 (1500, 85.19)
%                 (1600, 85.65)
%                 (1700, 86.08)
%                 (1800, 86.52)
%                 (1900, 86.89)
%                 (2000, 87.25)
%                 (2100, 87.61)
%                 (2200, 87.95)
%                 (2300, 88.24)
%                 (2400, 88.50)
%                 (2500, 88.78)
%                 (2600, 89.02)
%                 (2700, 89.30)
%                 (2800, 89.51)
%                 (2900, 89.75)
%                 (3000, 89.97)
%                 (3100, 90.20)
%                 (3200, 90.40)
%                 (3300, 90.61)
%                 (3400, 90.79)
%                 (3500, 90.95)
%                 (3600, 91.12)
%                 (3700, 91.29)
%                 (3800, 91.43)
%                 (3900, 91.58)
%                 (4000, 91.72)
%                 (4100, 91.87)
%                 (4200, 92.02)
%                 (4300, 92.17)
%                 (4400, 92.30)
%                 (4500, 92.42)
%                 (4600, 92.55)
%                 (4700, 92.67)
%                 (4800, 92.79)
%                 (4900, 92.90)
%                 (5000, 93.01)
%                 (5100, 93.12)
%                 (5200, 93.23)
%                 (5300, 93.30)
%                 (5400, 93.38)
%                 (5500, 93.49)
%                 (5600, 93.58)
%                 (5700, 93.66)
%                 (5800, 93.74)
%                 (5900, 93.80)
%                 (6000, 93.87)
%                 (6100, 93.94)
%                 (6200, 94.03)
%                 (6300, 94.10)
%                 (6400, 94.19)
%                 (6500, 94.27)
%                 (6600, 94.37)
%                 (6700, 94.44)
%                 (6800, 94.51)
%                 (6900, 94.59)
%                 (7000, 94.67)
%                 (7100, 94.73)
%                 (7200, 94.80)
%                 (7300, 94.85)
%                 (7400, 94.91)
%                 (7500, 94.97)
%             };
%     \end{axis}
% \end{tikzpicture}


% % \end{tabular}
% % }
% % \caption{\label{fig:appearance} The relation between news appearance times and proportion of news articles. Each point (x, y) represents y \% of news articles appear less than x times within a training epoch.
% % }
% % \end{figure}


==> Tables/benchmark.tex <==
\newcommand{\mosmall}[1]{\texttt{\textcolor[HTML]{3E7A3E}{#1}}}  % acceptable color
\newcommand{\momedian}[1]{\texttt{\textcolor[HTML]{6C75D6}{#1}}}  % unacceptable color
\newcommand{\molarge}[1]{\texttt{\textcolor[HTML]{DB3636}{#1}}}  % unacceptable color

\begin{table}[t]

\centering
% \renewcommand\arraystretch{1.2}
\setlength\tabcolsep{4pt}

\resizebox{\linewidth}{!}{

\begin{tabular}{llllllll}
\toprule
 & \multicolumn{1}{c}{ID-based} & \multicolumn{3}{c}{End-to-end Text-based} & \multicolumn{1}{c}{Pretrain-Finetune} & \multicolumn{2}{c}{\model{}} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-6} \cmidrule(lr){7-8} 
 & Null & Pooling & CNN & Attention & BERT & BERT & MFT \textit{(ours)} \\
\midrule
Null & \makecell[l]{DIN\\\mosmall{6.91M}} & \makecell[l]{Text-DIN\\\momedian{28.59M}} & - & - & \makecell[l]{PLMNR-DIN\\\molarge{52.02M}} & \makecell[l]{BERT-DIN\\\mosmall{6.91M}} & \makecell[l]{MFT-DIN\\\mosmall{6.91M}} \\
Pooling & \makecell[l]{DCN\\\mosmall{5.32M}} & \makecell[l]{Text-DCN\\\momedian{27.01M}} & - & - & \makecell[l]{PLMNR-DCN\\\molarge{50.44M}} & \makecell[l]{BERT-DCN\\\mosmall{5.32M}} & \makecell[l]{MFT-DCN\\\mosmall{5.32M}}\\
\makecell[l]{Additive\\Attention} & \makecell[l]{ID-NAML\\\mosmall{2.36M}} & - & \makecell[l]{NAML\\\momedian{26.41M}} & - & \makecell[l]{PLMNR-NAML\\\molarge{47.48M}} & \makecell[l]{BERT-NAML\\\mosmall{2.36M}} & \makecell[l]{MFT-NAML\\\mosmall{2.36M}}\\
GRU & \makecell[l]{ID-LSTUR\\\mosmall{12.99M}} & - & \makecell[l]{LSTUR\\\momedian{32.31M}} & - & \makecell[l]{PLMNR-LSTUR\\\molarge{51.02M}} & \makecell[l]{BERT-LSTUR\\\mosmall{12.99M}} & \makecell[l]{MFT-LSTUR\\\mosmall{12.99M}} \\
Attention & \makecell[l]{ID-NRMS\\\mosmall{5.32M}} & - & - & \makecell[l]{NRMS\\\momedian{30.55M}} & \makecell[l]{PLMNR-NRMS\\\molarge{50.43M}} & \makecell[l]{BERT-NRMS\\\mosmall{5.32M}} & \makecell[l]{MFT-NRMS\\\mosmall{5.32M}} \\
Transformer & \makecell[l]{BST\\\mosmall{25.20M}} & \makecell[l]{Text-BST\\\momedian{46.89M}} & - & - & \makecell[l]{PLMNR-BST\\\molarge{70.32M}} & \makecell[l]{BERT-BST\\\mosmall{25.20M}} & \makecell[l]{MFT-BST\\\mosmall{25.20M}} \\
\bottomrule
\end{tabular}

}

\caption{Methods and variants that will be benchmarked and compared. The first row is a set of different news encoders, and the first column is a set of different user encoders.\label{tab:benchmark}}
\end{table}
